G4G:A Generic Framework for High Fidelity Talking Face Generation with Fine-grained Intra-modal Alignment

Despite numerous completed studies, achieving high fidelity talking face generation with highly synchronized lip movements corresponding to arbitrary audio remains a significant challenge in the field. The shortcomings of published studies continue to confuse many researchers. This paper introduces G4G, a generic framework for high fidelity talking face generation with fine-grained intra-modal alignment. G4G can reenact the high fidelity of original video while producing highly synchronized lip movements regardless of given audio tones or volumes. The key to G4G's success is the use of a diagonal matrix to enhance the ordinary alignment of audio-image intra-modal features, which significantly increases the comparative learning between positive and negative samples. Additionally, a multi-scaled supervision module is introduced to comprehensively reenact the perceptional fidelity of original video across the facial region while emphasizing the synchronization of lip movements and the input audio. A fusion network is then used to further fuse the facial region and the rest. Our experimental results demonstrate significant achievements in reenactment of original video quality as well as highly synchronized talking lips. G4G is an outperforming generic framework that can produce talking videos competitively closer to ground truth level than current state-of-the-art methods.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% \textbf{1.当前talking face generation的市场需求和行业现状；}
% 2.当前相关技术覆盖到了哪些方面；
% 3.当前技术存在哪些缺陷和局限性；
% 4.我们的文章为了解决哪些问题，提出了什么框架，主要组成部分和特征是哪些（罗列）？\

Audio-driven talking face generation has emerged as a crucial and fundamental component in the rapidly evolving virtual world. This technology finds widespread application in video dubbing for multilingual situations\cite{zhou2019talking,Gao2021VisualVoice}, movie animations\cite{thies2020neural,ren2021pirenderer}, and communication aids for individuals with hearing difficulties who rely on lip-reading\cite{liu2023moda,wang2023seeing}. The primary objective of talking face generation is to synthesize a high-fidelity video of a target identity with lip movements synchronized to arbitrary audio\cite{ling2010analysis}, thereby significantly reducing video production costs in this industry.

Talking face generation methods can be broadly classified into two categories based on their training pipeline and data requirements: person-specific and person-generic. While person-specific methods can generate photo-realistic talking face videos, they require re-training or fine-tuning the model with target-speaker's videos, which is not practical in real-world scenarios\cite{zhong2023identity,ma2023styletalk}, where hand gestures and body motions are also important. Therefore, the generation of person-generic talking face videos has garnered more research interest in the field. To achieve results that are as close as possible to the ground truth for person-generic methods, we focus on intra-modal features alignment between the generated talking face and the speaker's original video, as well as inter-modal features alignment between the generated lip movements and the given driving audio.

Person-generic talking face generation poses three major challenges: 1) generating a photo-realistic talking face with the same facial texture and expressions as the speaker's source video, 2) ensuring that the generated lip movements are coherent with the audio, and 3) producing a high-fidelity talking face video. To address these issues, many methods leverage prior-based preprocessing as an intermediate representation. Prajwal et al.\cite{prajwal2020lip} used the lower-half masked input video as a pose prior, while Zhong et al.\cite{zhong2023identity} devised a Transformer-based landmark generator to obtain lip and jaw landmarks as prior appearance. Zhang et al.\cite{zhang2023dinet} performed spatial deformation on feature maps of reference images and source images. However, they directly fused the features of source images and reference images with simple operations without modeling the underlying correlation between them. Zhou et al.\cite{zhou2021pose} separately considered speech content-related landmarks and speaker identity-related landmarks for unseen subjects. Park et al.\cite{park2022synctalkface} proposed audio-lip memory to enforce fine-grained audio-visual coherence. However, the translation from audio to generated face is a dynamic matching process, considering that the same pronunciation may correspond to multiple lip movements according to the source video's expression and facial shapes. These problems demonstrate that these methods struggle with synthesizing synchronized lip movements with the given audio\cite{liang2022expressive, zhang2022meta}.

To cope with the above problems, we devised a novel alignment-deformation framework composed of a fine-grained feature alignment network, a multi-scale perceptional network and a deformation fusion network. The goal of our framework is to generate the talking face with same facial textual and face shape as the source video and coherent lip movements according to the phonetic motion of the audio\cite{guo2021ad}. Specifically, we propose a fine-grained alignment network which includes the intra-modality alignment network and inter-modality alignment network. The intra-modality alignment network utilize facial landmarks extracted from source video as extra supervision to align the generated talking face with the target person. The inter-modality alignment network utilized the aligned visual features to conduct matrix alignment with the audio features. The alignment methods helps to prevent the generated face deviate from the target face outline and to better capture the relationships between audio feature and visual feature. Then, we utilized multi-scale supervised adaptive spatial transformation network to deform the visual features under the guidance of audio and generate the deformed talking face under the supervision of multi-scale mask. Our method prevents the generation from scratch, which can better protect the texture of the mouth area and the face contour. Additionally, due to the face artifacts caused by mask, we need a face fusion network to smooth the face contour. Extensive experiments demonstrate that our method produces more high-fidelity and lip-synced talking face videos. Our main contributions are summarized as follows:
\begin{itemize}
    \item We design a comprehensive network which includes an intra-modality alignment and an inter-modality alignment modules. The fine-grained align network could employ the alignment of visual features and audio features with different granularity.
    \item We propose an align-deformation network composed of a diagonal matrice- based fine-grained alignment network to address the person-generic talking face generation tasks under the guidance of prior landmark and audio.
    \item We introduce a multi-scale supervised adaptive spatial transformation network, which can move pixels into appropriate locations under the guidance of audio and multi-scale masks to better protect the texture of the mouth area and the face contour.
    \item Extensive experiments are conducted on LRS2\cite{afouras2018deep} and HDTF\cite{zhang2021flow} dataset, demonstrated the superiority of our method compared to other state-of-art methods in aspect of high-fidelity and lip synchronization. 
    
\end{itemize}


% id vector and facial landmarks extracted from source video as extra supervision to align the generate talking face with the target person. Then we utilize the aligned visual features to conduct matrix alignment with the audio features.
%-------------------------------------------------------------------------

% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}



% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Overview of our alignment-deformation framework}
%    \label{fig:framework}
% \end{figure}

% \subsection{Miscellaneous}



% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/2_Related.tex <==
\section{Related Work}

% 1.在高清画质生成方面的工作覆盖，仍存在的缺陷和局限性，包括画质模糊、连续帧闪烁、融合框痕迹等；
% 2.音频和图像编解码和对齐方面的工作覆盖，仍存在的缺陷和局限性；
\begin{figure*}[htbp]
  \centering
   \includegraphics[width=0.9\linewidth]{Figure/figure1.png}
   \caption{Overview of our alignment and deformation framework.}
   \label{fig:framework}
\end{figure*}

\subsection{High Quality Talking Face Generation}
In few-shot talking face generation, recent works leverage intermediate facial representations, including facial landmarks\cite{biswas2021realistic,chen2020talking} and 3DMM\cite{blanz2023morphable,mildenhall2021nerf} to split a pipeline into two phases. The first phase produces facial parameters of motion field from driving audio\cite{wu2023speech2lip,hong2023implicit}. The second phase transforms the facial parameters into talking face videos\cite{zhang2023metaportrait,wang2022one}. Directly learning a mapping function from audio to the head motion in the reference face image encountered the problem of ambiguity\cite{nagrani2020disentangled}, which results to misaligned properties of image generation, such as misalignment of the generated face id and lip motion with the driving audio. Some works\cite{zhang2023dinet,jang2023s} ignore this problem, leading to synthesize talking face videos with obvious artifacts and flaw. For example, thanks to the strong supervised information of SyncNet\cite{chung2017out}, Wav2Lip\cite{prajwal2020lip} has good generalization and good synchronization of lips motion and audio. Since no fine-grained feature alignemnt in the latent space, a sudden change of the mouth movement could lead to discoordination with the driving audio. There are also some person-generic methods which can synthesize talking face videos for unseen speakers\cite{liu2022semantic,ji2022eamm}. PC-AVS\cite{zhou2021pose} has achieved for arbitrary-subject audio-driven talking face generation by devising an implicit low-dimension pose code and learning the intrinsic synchronization between audio-visual modalities to modularize audio-visual representations. However, it is not enough to achieve feature alignment between different modalities with some naive operations.

\subsection{Audio and Visual Features Alignment}

Audio and visual alignment aims to find the spatial correlation and temporal coherence between audio and visual feature. In the context of talking face generation task, SyncNet\cite{chung2017out} utilized the contrastive loss variants that turned out to be a strong alternative for its effectiveness on cross-modal tasks. Zhu et al.\cite{zhu2018arbitrary} presented asymmetric mutual information estimator and dynamic attention block by selectively focusing the lip area of the input image to further enhance lip synchronization. Some work\cite{wang2023lipformer,liu2023moda} on cross modal learning applied multi-way matching loss that considered intra-class pairs as well as inter-class pairs. MakeItTalk\cite{zhou2020makelttalk} proposed to combine the LSTM and self-attention mechanisms to align the speaker's face landmark and audio and jointly learned audio-visual speech separation and cross-modal speaker embeddings. Se et al.\cite{park2022synctalkface} introduced audio-lip memory that brought in visual information of the mouth region corresponding to input audio and stored lip motion features in value memory and aligns them with corresponding audio features. Zhong et al.\cite{zhong2023identity} proposed an alignment module to register reference images and their features with target face pose and expression. Although the existing methods use different alignment networks at different stages, they do not consider the underlying feature correlation of different granularity between the same modality and different modality\cite{liang2022expressive,qi2023difftalker}.
%-------------------------------------------------------------------------

%-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

%-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.


% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }




==> sec/3_Method.tex <==
\section{Method}
Given an audio sequence and a source video, we aim to generate a high-fidelity lip-synced talking face video. The framework of our method is depicted in Fig 1. which is composed of two stages. The first stage includes an intra-modality alignment network which takes the landmarks of the target speaker's face and lower-half occluded face as input and an inter-modality alignment network which takes the aligned visual and audio feature as input to predict audio-guided visual feature. The second stage consists of an multi-scaled supervised adaptive spatial transformation network to deform the aligned visual features and generate the deformed talking face under the supervision of multi-scale mask. Additionally, a face fusion network is utilized to smooth the face contour and clear artifacts of generated face frames. We detail these three parts in the following.
\subsection{Fine-Grained Feature Alignment}
\subsubsection{Intra-modality Feature Alignment}
Given a source image $I_{s} \in \mathbb{R}^{3 \times H \times W}$, an audio embedding  $A \in \mathbb{R}^{16 \times 80}$, five reference images $I_{r} \in \mathbb{R}^{15 \times H \times W}$ and a prior landmarks $L_{r} \in \mathbb{R}^{1 \times H \times w}$. $A$ is input into an audio encoder to extract audio feature $a$. $I_{s}$, $I_{r}$, $L_{r}$ are input into three different feature encoders to extract source embedding $i_{s}$, $i_{r}$ and $l_{r}$ respectively. $a, i_{s}, i_{r}, l_{r} \in \mathbb{R}^{d}$ (d is the dimension of feature). This process is formulated as follows:
\begin{align}
a&=E_{a}(A),\\
i_{s}&=E_{s}(I_{s}),\\
i_{r}&=E_{r}(I_{r}),\\
l_{r}&=E_{s}(L_{r}),
\end{align}
We utilize the $1D$ convolution layers to concat the feature $i_{s}$ and $i_{r}$ to get the feature $\overline{i}_s$, then we input the feature $\overline{i}_s$ and $l_{r}$ into the intra-modality alignment network. Since our task is to preserve the facial attribute information in $\overline{i}_s$ and identity information of $l_{r}$. we need to align the visual feature of lower-half occluded face with the landmark feature of the reference image. So we should conduct modifications on the feature  $\overline{i}_s$ and to learn implicitly which part of feature $\overline{i}_s$ should be changed or preserved. We ustilzie the combination of Residual Block and Adaptive Instance Normalization(AdaIN)\cite{huang2017arbitrary} as the intra-modality alignment network. Here $\mu(\overline{i}_s)$ and $\sigma(\overline{i}_s)$ is the channel-wise mean and standard deviation of the feature $\overline{i}_s$. $\dot{\sigma}, \dot{\mu}$ are two parameters of full connected layers generated from $l_{r}$. 
\begin{equation}
    AdaIN(\overline{i}_s, l_{r})=\dot{\sigma}\frac{\overline{i}_s-\mu(\overline{i}_s)}{\sigma(\overline{i}_s)}+\dot{\mu}
\end{equation}
By the intra-modality alignment network, we get the aligned visual feature $\overline{i}_{align}$. 
\subsubsection{Inter-modality Feature Alignment}
Through the visual feature alignment, we can retain the facial attribute information and identity information of target person, which could make our framework person-generic and can not be covered by high
-frequency facial attributed of the trained dataset. Inspired by the work\cite{radford2021learning,li2021align}, we utilized two different modalities which are audio feature $a$ and aligned visual feature $\overline{i}_{align}$ to conduct contrastive learning. We conduct matrix dot to get the score matrix between the row-wise aligned visual feature and the column-wise audio feature to align different modality feature. By contrast to the similarity score of a batch of positive and negative auido-visual samples, we could be able to distinguish the negative samples closest to the positive samples. The calculation process is summarized as below.
\begin{align}
    s(V,A)&=g_{v}(\overline{i}_{align})^{T} \cdot g'_{a}(a'),\\
    s(A,V)&=g_{a}(a)^{T}\cdot g'_v(\overline{i'}_{align})
\end{align}

\begin{align}
    p^{v2A}(V)&=\frac{exp(s(V,A)/\tau)}{\sum_{i=1}^{N}exp(s(V,A)\tau)}\\
    p^{A2V}(A)&=\frac{exp(s(A,V)/\tau)}{\sum_{i=1}^{N}exp(s(A,V)\tau)}
\end{align}

where the $g_v$ represents the visual encoder, $g_a$ represents the audio encoder, $S(V,A)$ represents the score value of the transpose of visual feature and the audio feature, $S(A,V)$ represents the score value of the transpose of audio feature and the visual feature. Foe each visual image and audio, we calculate the softmax-normalized visual-to-audio and audio-to-visual similarity as $p^{v2A}(V)$ and $p^{A2V}(A)$

\subsection{Multi-Scale Perception Supervision}
In this part, we concatenate the aligned visual feature $F_{aligned}^{v}$ and the aligned audio feature  $F_{aligned}^{a}$ to get the feature $\overline{F}_{aligned}$. Considering that the masks of different sizes can affect the deformation coefficient of the feature channel, in order to obtain feature combinations of different granularity, we utilize the multi-scale mask as supervision of spatial adaptive deformation operators to deform the reference feature $F_{ref}$. We deform the feature with adaptive spatial layouts by computing different affine deformed coefficients in different feature channel. We utilized the fully-connected layers to compute the coefficients of rotation $R={\theta^{c}}_{c=1}^{256}$, translation $T_x={t^{c}_{x}}_{c=1}^{256}/T_y={t^{c}_{y}}_{c=1}^{256}$ and scale $S={s^{c}}_{c=1}^{256}$. These adaptive affine deformed coefficients are used to do affine transformations on $F_{ref}$.
\begin{align}
\setlength{\arraycolsep}{1.4pt}
\left[\begin{array}{c}
\hat{x}_c \\
\hat{y}_c
\end{array}\right]=\left[\begin{array}{ccc}
s^c \cos \left(\theta^c\right) & s^c\left(-\sin \left(\theta^c\right)\right) & t_x^c \\
s^c \sin \left(\theta^c\right) & s^c \cos \left(\theta^c\right) & t_y^c
\end{array}\right]\left[\begin{array}{c}
x_c \\
y_c \\
1
\end{array}\right]
\end{align}
where $x_c,y_c$ represent the original pixel coordinates,  $\hat{x}_c,\hat{y}_c$ denote the deformed pixel coordinates. $c \in [1,256]$ represents the $c-th$ channel in $F_{ref}$. Then we get the deformed feature $F_d$. Then we concatenate the source image feature $F_s$ and deformed feature $F_d$ in feature channel. Then a feature decoder is used to generated the talking face images. 

Since the generated face may include small portions of background rectangle and artifacts caused by the lower-half occluded mask. We composite the generated face with the Gaussian-smoothed face mask. Then we utilized a blend net to synthesize harmonized final output image after the composition operation.
The blend net is fusion and amending the final face image instead of generation by predicting the pixel residual.

\subsection{Training Objectives}
In training stage, we use three kind of loss functions to train our framework, including facial attribute loss, perception loss, GAN loss, L1 reconstruction loss and contrastive learning loss.

% \begin{equation}
%     AdaIN(\overline{i}_s, l_{r})=\dot{\sigma}_{r}\frac{\overline{i}_s-\mu(\overline{i}_s)}{\sigma(\overline{i}_s)}+\dot{\mu}_{r}
% \end{equation}
we utilize the facial attribute loss to constrain the distance between source feature $\overline{i}_s$ and the reference landmark feature $l_{r}$. We are using the cosine similarity to calculate the distance, which can be written as:
\begin{align}
\mathcal{L}_{v}=1-\frac{\overline{i}_s \cdot l_{r}}{\left\|\overline{i}_s\right\|_{2}\left\|l_{r}\right\|_{2}}
\end{align}

 We compute the perception loss in two image scale. Specifically, we downsample the output image and real image into $\hat{I}_{o} \in \mathbb{R}^{3\times \frac{H}{2} \times  \frac{W}{2}}$ and  $\hat{I}_{r} \in \mathbb{R}^{3\times \frac{H}{2} \times  \frac{W}{2}}$ . Then, paired images ${I_{o},I_{r}}$ and ${\hat{I}_{o},\hat{I}_{r}}$ are input into a pretrained VGG-19 network to compute the perception loss. The perception loss is written as

\begin{small} 
\begin{equation} 
\mathcal{L}_p=\sum_{i=1}^N \frac{\left\|V_i\left(I_o\right)-V_i\left(I_r\right)\right\|_{1}+ \left\|V_i\left(\hat{I}_o\right)-V_i\left(\hat{I}_r\right)\right\|_{1}}{2 N W_i H_i C_i}
\end{equation} 
\end{small}

% \begin{equation}

% \mathcal{L}_p=\sum_{i=1}^N \frac{\left\|V_i\left(I_o\right)-V_i\left(I_r\right)\right\|_{1}+ \left\|V_i\left(\hat{I}_o\right)-V_i\left(\hat{I}_r\right)\right\|_{1}}{2 N W_i H_i C_i}
% \end{equation}

where $V_{i}$ represents the i-th layer in VGG-19 network. $W_{i}H_{i}C_{i}$ is the feature size in i-th layer.

We use effective LS-GAN loss in our method. The GAN loss is written as
\begin{align}
\mathcal{L}_D&=\frac{1}{2} E\left(D\left(I_r\right)-1\right)^2+\frac{1}{2} E\left(D\left(I_o\right)-0\right)^2 \\
\mathcal{L}_G&=E\left(D\left(I_o\right)-1\right)^2 .
\end{align}
where G represents the generator and D denotes discriminator. We use the GAN loss on both single frame and five consecutive frames, the GAN loss is described as $\mathcal{L}_{GAN}=\mathcal{L}_{G}+\mathcal{L}_D$

we use L1 reconstruction loss to minimize the margin between the source feature with multi-scale mask and the reference feature, which is described as follows:
\begin{align}
\mathcal{L}_r=\frac{1}{N}\sum_{i=1}^{N}(\left\|I_{s}-I_{r}\right\|_{1})
\end{align}

To further improve the synchronization performance, we introduce a pre-trained sync expert network to boost the model's performance in lip motion and audio sunchronization. The unsynced audio-image pairs are exploited to construct the contrastive loss. The distance of synced audio-image pairs is expected to be closer while the unsynced audio-image pairs should be farther. Thus we utilize the cross-entropy to represent the contrastive learning loss, which is defined as follows:
 % p^{v2A}(V)

\begin{small} 
\begin{equation} 
    \mathcal{L}_{con}=\frac{1}{2}\mathbb{E}_{V,A}[H(y^{v2a}(V),p^{v2A}(V))+\\
    H(y^{a2v}(A),p^{a2v}(A))]
\end{equation} 
\end{small}

To summarize, the training loss for the alignment-deformation framework can be formulated as follows:
\begin{align}
\mathcal{L}==\lambda_{v}\mathcal{L}_v+\lambda_{p}\mathcal{L}_p+\lambda_{GAN}\mathcal{L}_{GAN}+\lambda_{r}\mathcal{L}_r+\lambda_{con}\mathcal{L}_{con}
\end{align}

We set $\lambda_{v}$=1, $\lambda_{p}$=2, $\lambda_{GAN}$=3, $\lambda_{r}$=4, $\lambda_{con}$=5 in our experiment respectively.
% \subsubsection{Inter Modality Feature Alignment}

% \subsubsection{Loss Function for Feature Alignment}

% \subsection{Adaptive transformation Network}

% \subsubsection{Adaptive Affine Transformation Module}

% \subsubsection{Face fusion}

% \subsubsection{Loss Function}

==> sec/4_Experiments.tex <==
\section{Experiments}
In this section, we first detail our datasets, evaluating metrics and implementation details. Then we compare our quantitative and qualitative results with other state-of-art methods. Next, we conduct ablation studies to analyze our significant module. Finally, a user study is conducted to validate our method.

\subsection{Datasets}

We conduct experiments on two high-fidelity talking face datasets: HDTF dataset\cite{zhang2021flow} and  LRS2 dataset\cite{afouras2018deep}.

\textbf{HDTF dataset.} HDTF dataset contains about 400 wild videos collected with 1080P resolution. We randomly select 20 videos for testing in our experiments.

\textbf{LRS2 dataset.} The dataset consists of 48164 video clips from outdoor shows on BBC television. Each video is accompanied by an audio corresponding to a sentence with up to 100 characters. We split the training and testing sets into 8:2. We sample 45 videos for testing.


\subsection{Evaluating Metrics}
\textbf{Visual Quality Metrhics.} We use Peak Signal-to-Noise Ratio (PSNR) and Structured similarity (SSIM)\cite{wang2004image} to measure the similarity between generated and ground-truth images. Learned Perceptual Image Patch Similarity (LPIPS)\cite{zhang2018unreasonable} and Frechet Inception Distance (FID)\cite{heusel2017gans} are employed to measure the feature-level similarity. We utilized the Lip-Sync Error-Distance (LSE-D) and Lip-Sync Error-Confidence (LSE-C) to measure the lip-sync accuracy.

\subsection{Implementation Details}
In data processing, all videos are resampled in 25 fps. We extract 68 facial landmarks from openface and crop and resize all faces into 416 $\times$ 320 resolution. The mouth region covers 256 $\times$ 256 resolution in resized facial image. We calculate Mel-spectrogram feature from audios using a window size of 800 and sample rate of 16khz. The learning rate is set to 0.0001. The batch size is set to 3 on a A100 GPU.Our method realized photo-realistic talking face on 1080P videos.


\subsection{Comparison with State-of-the-Art Method}
We compare our method with state-of-art talking face generation including Wav2Lip\cite{prajwal2020lip}, VideoRetalking\cite{cheng2022videoretalking}, DiNet\cite{zhang2023dinet} and IPLAP\cite{zhong2023identity}. Wav2Lip uses an encoder-decoder model learned via a lip expert discriminator to produce talking face videos. VideoRetalking generates emotional talking face video using the canonical expression template using the expression editing network. Dinet develops a deformation inpainting network for realistic face visually dubbing on high-resolution videos by conducting spatial deformation on feature maps of reference facial images to inpaint mouth. IPLAP proposes a two-stage framework composed of an audio-to-landmark generator and a landmark-to-video rendering model to address the person-generic talking face generation task under the guidance of prior landmark and appearance information.

\textbf{Quantitative comparisons.} We conduct a quantitative comparison of talking face generation that the input audio comes from the source video. Our methods are conducted on  LRS2 and HDTF datasets. As shown in Table~\ref{table:tab1}, our model generates talking faces with the highest PSNR, SSIM and LPIPS on both datasets in the evaluation of visual quality.
Especially in SSIM and LPIPS, our method is significantly better than other methods by large margins. The SSIM of our method is 10.28\% and 7.32\% larger than that of the second-best method, Wav2Lip on LRS2 and HDTF datasets. The reason is that our method can effectively leverage the landmarks of reference images to align the personalized facial attributes of any generic person, while other methods tend to generate the average facial attributes of training dataset. In the evaluation of audio-visual synchronization, our method is better than other methods. One possible reason is that our method aligned the lip movement to the audio and make the lip syncronization more accurate.

\begin{table*}[htbp]
\caption{The quantitative comparison with other methods on the talking face generation.$\uparrow$ indicates higher is better while $\downarrow$ indicates lower is better.}
\label{table:tab1}
\centering
\begin{tabular}{c|c|cccccc}
\hline \multirow{2}{*}{ Method } & \multirow{2}{*}{ Dataset } & \multicolumn{6}{c}{ Reconstruction } \\
\cline { 3 - 8 } & & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & MSE $\downarrow$ &  LSE-D$\downarrow$ & LSE-C $\uparrow$  \\
\hline  
Wav2Lip\cite{prajwal2020lip}& &27.9359 & 0.8935 & 0.1455 & 0.0017 & 7.0138 & 8.3739  \\
VideoRetalking\cite{cheng2022videoretalking} & & 23.8450 & 0.8479 & 0.1262 & 0.0046 & 7.2773 & 7.5827  \\
DiNet\cite{zhang2023dinet} &HDTF  & 23.7150 & 0.8558 & 0.1017 & 0.0045 & 8.0256 & 7.0689  \\
IPLAP\cite{zhong2023identity} && 27.9556 & 0.9088 & 0.0918 & 0.0018 & 8.2667 & 6.3498  \\
Ours & & $\mathbf{27.5560}$ & $\mathbf{0 . 9 083}$ & $\mathbf{0 . 0904}$ & $\mathbf{0.0020}$ & $\mathbf{7.8920 }$ & $\mathbf{7.3381}$ \\
\hline 
Wav2Lip\cite{prajwal2020lip} & & 28.4655 & 0.8928 & 0.1542 & 0.0014 & 7.0256 & 8.2106  \\
VideoRetalking\cite{cheng2022videoretalking} & & 25.8770 & 0.8430 & 0.1451 & 0.0026 & 7.0523 & 7.5366 \\
DiNet\cite{zhang2023dinet} &LRS2 & 26.8306 & 0.8765 & 0.0966 & 0.0022 & 8.1542 & 6.6632  \\
IPLAP\cite{zhong2023identity} & & 27.3878 & 0.8798 & 0.1106 & 0.0020 & 9.3604 & 4.8714  \\
Ours & & $\mathbf{27.0606}$ & $\mathbf{0 . 9101}$ & $\mathbf{0 . 0846}$ & $\mathbf{0.0020}$ & $\mathbf{8.5688}$ & $\mathbf{6.5064}$  \\
\hline
\end{tabular}

\end{table*}

\begin{figure*}[htbp]
  \centering
   \includegraphics[width=0.9\linewidth]{Figure/cvprexp.pdf}
   \caption{Qualitative comparisons with state-of-art person-generic methods on LRS2 dataset\cite{afouras2018deep} and HDTF\cite{zhang2021flow} }
   \label{fig:qualitative}
\end{figure*}
\textbf{Qualitative comparisons.} We first compare with state-of-the-art works in qualitative comparisons. Figure~\ref{fig:qualitative} illustrates the qualitative results.It shows that our method generates the highest quality video with mouth shapes that best match the ground truth, meanwhile the teeth shape and facial textual are photo-realistic. Wav2Lip only utilized the lower-half mask to supervise the mouth area and a lip-sync expert to enhance lip-sync. It generated talking face with lower-quality teeth and facial artifacts. The main reason is that wav2lip utilizes networks to dierctly generate pixels in mouth region, making networks easily neglect textural details. The Dinet just conducted the simple operation on feature, they did not consider the underlying feature correlation. It generated talking face with neural expression and unclear mouth texture. VideoRetalking generated vivid expression and photo-realistic facial texture, but it did not consider the alignment of audio and visual feature, so the generated video produces lip jitter and lip motion inconsistency. The IPLAP generated the talking face by fusing the prior landmark information with the audio features. But they can not consider the facial texture and teeth shape. Although they
are trained on high resolution videos. Our G4G network align the visual feature and audio feature and deforms existing facial pixels into appropriate locations of mouth region rather than generate from scratch, thus achieves more photo-realistic and natural-looking results.

\begin{table}[htbp]
\caption{The ablation study on our components. $\uparrow$ indicates higher is better while $\downarrow$ indicates lower is better.}
\label{table:tab2}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\hline Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & MSE $\downarrow$ & LSE-D $\downarrow$ &LSE-C $\uparrow$ \\
\hline w/o alignment & 23.7250 & 0.8557 & 0.1027 & 0.0042 & 8.0251 & 7.0682 \\
w/o supervision & 27.6478 & 0.9160 & 0.0783 & 0.0019 & 7.7244 &7.4636 \\
w/o fusion & 25.7960 & 0.8746 & 0.1082 & 0.0030 & 7.9698 & 7.3311\\
Ours & $\mathbf{27.5560}$ & $\mathbf{0 . 9 083}$ & $\mathbf{0 . 0904}$ & $\mathbf{0.0020}$ & $\mathbf{7.8920 }$ & $\mathbf{7.3381}$ \\
\hline
\end{tabular}
}
\end{table}
\subsection{Ablation Study}
In this section, we conduct ablation experiments to validate the effect of each component in our G4G framework on the HDTF dataset. Specifically, we set three conditions: (1)
Ours w/o diagonal fine-grained alignment: we remove the alignment operation in our whole model and use the convolution operation to replace it. (2) Ours w/o multi-scale perception supervision. (3) Ours w/o fusion network.
\begin{figure}[htbp]
  \centering
   \includegraphics[width=0.9\linewidth]{Figure/cvpr_ablation.pdf}
   \caption{Qualitative comparisons with ablation study on HDTF\cite{zhang2021flow} datasets.}
   \label{fig:ablation}
\end{figure}

Figure~\ref{fig:ablation} illustrates the qualitative results of ablation experiments. In the condition of Ours w/o fine-grained alignment, the synthetic facial images have blurry mouth and mouth jitter. And due to without the large number of positive and negative sample pairs provided, the model training converges slower and need more iteration. Compared with w/o fine-grained alignment, our model improves LSE-C by about 19.5\% on LRS2 dataset. It indicates that it is important to align the intra-modality and inter-modality feature. In the condition of Ours w/o multi-scale perception supervision, the synthetic facial images have blur textural details of mouth area especially teeth. Compared with the w/o supervision, our model shows at least 26.5\% improvement on  LRS2 and 31.2\% improvement on HDTF dataset. These advantages confirm the positive effect of the multi-scale perception supervison. 
\subsection{User Study}
To validate the effect of our method qualitatively, we invite 20 persons from different work groups to evaluate the generated talking face videos of our method with the other four SOTA methods. Four videos are selected from each dataset for evaluation. Each participant is asked to rate the generated videos on visual quality, lip synchronization and video realness. Each metric ranges from 1 (pretty bad) to 5 (pretty good). The mean opinion scores of rating values can be observed on Table~\ref{table:tab3}. Our method gets the best rating score from participants on three indexes. Specifically, the mean opinion scores of our method is 8.6\%, 8.9\% and 17.9\% higher than that of the second best method on visual quality, lip synchronization and video realness respectively.

\begin{table}[htbp]
\caption{User study about video generation quality on }
\label{table:tab3}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c}
\hline Method & Visual Quality & Lip Synchronization & Video Realness \\
\hline 
Wav2Lip\cite{prajwal2020lip} & 2.92 & 3.34 & 3.51 \\
VideoRetalking\cite{cheng2022videoretalking} & 3.14 & 3.42 & 3.28 \\
DiNet\cite{zhang2023dinet} & 2.98 & 3.72 & 3.37 \\
IPTFP\cite{zhong2023identity} & 2.33 & 3.91 & 3.68 \\
Ours & $\mathbf{3 . 4 1}$ & $\mathbf{4 . 26}$ & $\mathbf{4 . 34}$ \\
\hline
\end{tabular}
}
\end{table}
\subsection{Limitation}
Our method achieves high-fidelity and highly synchronized talking face videos according to given audios, yet we still encounter several challenging conditions. Due to the training datasets mainly include straight head pose videos, so our G4G framework will have some artifacts in generating image sequences at large angle of head pose. In addition, the quickly changed background and illumination as well as movements can also bring some challenges in the final results. Further researches are in process, more results will be published soon.


% \subsection{Experimental Settings}

% \textbf{Implementation Details.}
% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.
% \textbf{Dataset.}
% \textbf{Comparison Methods}
% \subsection{Evaluation Metrics}
% \subsection{Quantitative Comparison}
% \subsection{Qualitative Comparison}
% \textbf{User Study.}
% \textbf{Visualization of Generated Videos}
% \subsection{Ablation Study}

% \textbf{Effectiveness of Intra Modality Feature Alignment}

% \textbf{Effectiveness of Inter Modality Feature Alignment}

% \textbf{Reference Images Warping}
% \textbf{\textbf{Reference Images Warping}}
% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.

% \subsubsection{Inter Modality Feature Alignment}

==> sec/5_conclusion.tex <==
\section{Conclusion}
In this paper, we proposed a generic framework, named G4G, for high fidelity and highly synchronized video generation. It includes a diagonal fine-grained alignment network and a multi-scale supervision and adaptive spatial transformation network to realize high-fidelity talking face generation in multi-scale details. The fine-grained alignment network is designed to perform intra-modality alignment and inter-modality alignment to preserve the face ID, attributes and rich textural details of the source images corresponding to arbitrary given audio. The multi-scale supervised adaptive spatial transformation network is utilized to perform the spatial deformation of mouth shape and head pose to achieve very high fidelity of generated videos. Series of experiments in our study show that our G4G framework is capable of preserving the source character identity, skin textures and details close to ground truth. Meanwhile, our method could generate highly synchronized lip movements corresponding to arbitrary given audio. This method outperforms the existing person-generic methods. Yet we still encountering challenges and more researches are being carried out and will be published soon.



